Universal Correspondence Network

We present a deep learning framework for accurate visual correspondences and demonstrate its effectiveness for both geometric and semantic matching, spanning across rigid motions to intra-class shape or appearance variations. In contrast to previous CNN-based approaches that optimize a surrogate patch similarity objective, we use deep metric learning to directly learn a feature space that preserves either geometric or semantic similarity. Our fully convolutional architecture, along with a novel correspondence contrastive loss allows faster training by effective reuse of computations, accurate gradient computation through the use of thousands of examples per image pair and faster testing with $O(n)$ feed forward passes for $n$ keypoints, instead of $O(n^2)$ for typical patch similarity methods. We propose a convolutional spatial transformer to mimic patch normalization in traditional features like SIFT, which is shown to dramatically boost accuracy for semantic correspondences across intra-class shape variations. Extensive experiments on KITTI, PASCAL, and CUB-2011 datasets demonstrate the significant advantages of our features over prior works that use either hand-constructed or learned features.

==> evaluations.tex <==
\subsection{Essential Matrix Decomposition}

Since we can establish correspondences, we can find essential matrix to estimate the translation and rotation of the camera. To refresh the readers of the pipeline, we will briefly describe in this section.

First, we select discriminative feature pairs using distance ratio test \cite{sift} and use RANSAC to find essential matrix.

Once we find the essential matrix, we can decompose the essential matrix into 4 different possible rotation/translation combinations and find the combination that has the most inliers to estimate the rotation and translation (up to scale).

Since we can estimate the translation of the camera up to scale, we can estimate the We computed the angle between the direction of translation and ground truth translation from GPS-IMU to measure the performance of the correspondences.

\subsection{Percentage of Correct Keypoints}

First proposed in \cite{pcp}, the Percentage of Correct Part (PCP) is used to evaluate the correspondence of non-rigid objects. For each predicted correspondence and corresponding ground truth correspondence, we find the deviation of the predicted correspondence. If the deviation is smaller than a certain threshold, we classify the prediction as correct.

Since the threshold is arbitrary, we vary the threshold from 1 pixel to 100 pixel and plot the accuracy on the y-axis.


==> implementation.tex <==
We usedf Caffe \cite{caffe} package for neural network implementation. Since the vanila caffe do not support layers we proposed, we addedk Correspondence Contrastive Loss Layer and Convolutional Spatial Transformer Layer to caffe. We varied few network structures that are based on VGG16 \cite{vggnet} and GoogLeNet \cite{googlenet}.

For each network variant, we added features subseequently. First, we enabled bilinear interpolation (BL) or hard negative mining (HN). Next, we added convolutional spatial transformer (ST).





==> network_architectures.tex <==
\scream{networks that are similar to GoogLeNet} \cite{googlenet} and VGGNet
\cite{vggnet}.

On Table~\ref{tab:conv3}, we list network architectures and
subsampling size. Since the network is applied
convolutionally, the input image size can be arbitrarily large. At the top, the
features are extracted at every 4th pixel. So the output size is $\frac{w}{4}
\times \frac{h}{4}$ if the input image size is $w \times h$. We name $d$ as the
downsampling factor (D. F.). The fovea size is the size of the image patch that
a neuron in the layer sees.

The final output of the network goes through a 1x1 convolution to reduce the
dimension of the final feature down to 128.

\begin{table}[htp]
  \scriptsize
    \begin{center}
    \begin{tabular}{|l|c|c|c|c|c|}
      \hline
      layer    & in kernel  & out dim & D.F. & fovea size & param \\ \hline \hline
      conv1\_1 & 3x3x3      & 64      & 1    & 3x3        & 1.7k  \\ \hline
      conv1\_2 & 3x3x64     & 64      & 1    & 5x5        & 37k   \\ \hline
      pool1\   & 3x3        & 64      & 2    & 7x7        & -     \\ \hline
      conv2\_1 & 3x3x64     & 128     & 2    & 11x11      & 73.7k \\ \hline
      conv2\_2 & 3x3x128    & 128     & 2    & 15x15      & 147.4k \\ \hline
      pool2\   & 3x3        & 128     & 4    & 19x19      & -      \\ \hline
      conv3\_1 & 3x3x128    & 256     & 4    & 27x27      & 295k   \\ \hline
      conv3\_2 & 1x1x256    & 128     & 4    & 27x27      & 32.7k  \\ \hline
    \end{tabular}
    \end{center}
    \caption{{\it conv3} network: The top layer {\it
        conv3\_2} is the feature layer. `in kernel` indicates $w \times h \times
      c_{in}$ and `out dim` indicates output dimension of the feature $c_{out}$.
      D.F. is the downsampling factor $d$. The dimension of the output
      activation is $w/d \times h/d \times c_{out}$. Fovea size is the
      dimension of input image patch that a neuron in the layer sees. Final
      output dimension of the feature is 128}
    \label{tab:conv3}
\end{table}

On the base structure, we can insert a convolutional spatial transformer to allow
the network to learn patch normalization. To make the spatial transformation
indepedent and not interfere with others, we inserted the convolutional
spatial transformer before the last convolution layer
(Table~\ref{tab:conv3-st-pool2}). Unlike the vanilla convolutional network, the
spatial transformer can vary the fovea size since it can apply arbitrary
scaling and rotation to the lower layer input, so we left the fovea size in the
Table~\ref{tab:conv3-st-pool2} empty.

We used the affine transformation, which has a greater degree of freedom than
rotation and scaling. Each output of the {\it pool2-param-2} layer corresponds to
$\theta_i$ in Eq.~\ref{eq:spatial-transformer-sampling}.

\begin{table}[htp]
  \scriptsize
    \begin{center}
    \begin{tabular}{|l|c|c|c|c|c|}
      \hline
      layer    & in kernel  & out dim & D.F. & fovea size & param  \\ \hline \hline
      conv1-1  & 3x3x3      & 64      & 1    & 3x3        & 1.7k   \\ \hline
      conv1-2  & 3x3x64     & 64      & 1    & 5x5        & 37k    \\ \hline
      pool1    & 3x3        & 64      & 2    & 7x7        & -      \\ \hline
      conv2-1  & 3x3x64     & 128     & 2    & 11x11      & 73.7k  \\ \hline
      conv2-2  & 3x3x128    & 128     & 2    & 15x15      & 147.4k \\ \hline
      pool2    & 3x3        & 128     & 4    & 19x19      & -      \\ \hline
      pool2-param-1 & 1x1x128 & 64    & -    & -          & 8.2k  \\ \hline
      pool2-param-2 & 1x1x64  & 4     & -    & -          & 260   \\ \hline
      conv3-1  & 3x3x128    & 256     & 4    & -          & 295k  \\ \hline
      conv3-2  & 1x1x256    & 128     & 4    & -          & 32.7k  \\ \hline
    \end{tabular}
    \end{center}
    \caption{{\it conv3-ST} network extends {\it conv3} network and incorporates the
      convolutional spatial transformer. The output of pool2 is used to \scream{}}
    \label{tab:conv3-st-pool2}
\end{table}

We also used GoogleNet for our experiments, which extends Network In Network
(NIN). To make the network densely extract features, we converted
the pool1 layer stride from 2 to 1 (Table~\ref{tab:nin-conv3}). The {\it NIN} layer
consists of indepdendent convolutions with 1x1, 3x3, 5x5 kernels and max
pooling, whose outputs are concatenated to form the final layer output.

\begin{table}[htp]
  \scriptsize
    \begin{center}
    \begin{tabular}{|l|c|c|c|c|c|}
      \hline
      layer   & in kernel  & out dim & D.F. & fovea size & param \\ \hline \hline
      conv1   & 7x7x3      & 64      & 2    & 7x7        & 9.4k  \\ \hline
      pool1   & 3x3x64     & 64      & 2    & 3x3        & -     \\ \hline
      nrm1    & -          & 64      & 2    & 7x7        & -     \\ \hline
      conv2-r & 1x1x64     & 64      & 2    & 7x7        & 4.1k  \\ \hline
      conv2   & 3x3x64     & 192     & 2    & 11x11      & 112k  \\ \hline
      nrm2    & -          & 192     & 2    & 11x11      & -     \\ \hline
      pool2   & 3x3        & 192     & 4    & 13x13      & -     \\ \hline
      NIN-3a  & 1x1, 3x3, 5x5 & 256  & 4    & 29x29      & 159k  \\ \hline
      NIN-3a  & 1x1, 3x3, 5x5 & 480  & 4    & 45x45      & 380k  \\ \hline
      conv3   & 1x1x480    & 128     & 4    & 45x45      & 61.5k \\ \hline
    \end{tabular}
    \end{center}
    \caption{{\it NIN-conv3} network: The network resembles the first 5 layers of
      GoogLeNet \cite{googlenet}. The network in network layer (NIN) consists
      of various convolutions and max pooling. Final output of the network is
      reduced to 128 dimensional features.}
    \label{tab:nin-conv3}
\end{table}

For the {\it NIN-conv3} network, we also applied the convolutional spatial
transformer before the final convolution layer to ensure that each
spatial transformation does not interfere with other trasformations. Please
refer to the supplementary material for the full network structures.


==> review.tex <==
% The method uses an energy based model that uses the given neighborhood
% relationships to learn the mapping function. For a family of functions G,
% parameterized by W, the objective is to find a value of W that maps a set of
% high dimensional inputs to the manifold such that the euclidean distance
% between points on the manifold, $D_W (X_1, X_2) = \|G_W (X_1) − G_W
% (X_2)\|^2$ approximates the “semantic similarity”of the inputs in input
% space, as provided by a set of neighborhood relationships. No assumption is
% made about the function $G_W$ except that it is differentiable with respect
% to $W$.

In this section, we will review a type of deep metric learniing method which is
referred to as a contrastive loss. First proposed in \cite{DrLIM,
faceVerification}, Contrastive Loss for learning a mapping $f(\mathbf{x}) \in
\mathbb{R}^d$ that preserves similarity.  Let $\mathbf{x}_i$ and $\mathbf{x}_j$
be image patches. If the patches are
similar (defined by the task), we want the mapping $f(\mathbf{x}_i)$ and
$f(\mathbf{x}_j)$ be closer to each other. If they are dissimilar patches, we
want them to be at least a margin $m$ apart. Let $y_{i,j} \in \{0, 1\}$ be an
indicator whether a pair is similar or dissimilar. The contrastive loss is
defined as,

\begin{align} \label{eq:contrastive-loss}
  L & = \frac{1}{2N} \sum_{(i, j)} y_{i,j} \|f(x_i) - f(x_j)\|^2 + (1 - y_{i,j})\max(0, m - \|f(x_i) - f(x_j)\|)^2
\end{align}

% To find correspondences, we want to learn a mapping that maps an input image
% patch into a vector in an embedding that preserve an underlying commonality.
% 
% For instance, if we want to find a mapping that is invariant to the perspective
% projection, the supervision we need is the correspondences of
% the same 3D points; if we want to find a semantically similar parts such as a
% beak of a bird, a left armrest on a chair, the correspondences are semantic
% part correspondences.
% 
% Using those correspondences, we can construct a set of constraints that defines an embedding.
% 
% constraints, the neural network is trained to find the mapping
% $\mathcal{F}$ that satisfies the constraints.
% 
% As mentioned in Sect.~\ref{sect:related-works}, there are two ways to define a
% metric embedding: contrastive loss and triplet loss. Constraints for
% contrastive loss (Eq.~\ref{eq:pairwise-constraints}) force distinct data
% instances to be mapped to the same points in the space if they are from the same
% class and maps other classes to be at least a margin apart from other classes.

% Constraints for triplet loss (Eq.~\ref{eq:triplet-constraint}) also encode the
% same constraints. A negative class has to be at least $m + \epsilon = m'$ away
% from the positive class.

% Constraint for triplet loss (Eq.~\ref{eq:triplet-constraint}) allows the data
% intances in the same class to be mapped to different points in the space but
% forces data from other classes to be at least margin further from the farthest
% distance between instances from the same class.

% Practical choice $\epsilon = 0$  for fast training makes the contrastive loss
% less flexible, but makes it easy to train. Triplet loss, however, allows more
% flexible space definition since the radius of the class is not determined by a
% hyper parameter, yet poses a difficulty in selecting the right triplet, which
% violates constraints to speed up training.
% 
% In this paper, we used the constraints Eq.~\ref{eq:pairwise-constraints}
% to define our embedding space.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A metric space can be defined using a set of constraints. We can construct a
% space that maps "semantically similar" instances to be close to each other and
% a dissimilar pair to be at least a margin apart. Such constraints can be
% mathematically represented as Eq.~\ref{eq:pairwise-constraints}.
% 
% \begin{equation} \label{eq:pairwise-constraints}
%   D(x, x_+) < \epsilon \quad \textrm{and} \quad D(x, x_-) > m
% \end{equation}

% The same embedding can be constructed using a triplet (positive and negative
% instance) using a constraint Eq.~\ref{eq:triplet-constraint} \cite{lmnn}.
% 
% \begin{equation} \label{eq:triplet-constraint}
%   D(x, x_+) + m' < D(x, x_-)
% \end{equation}

% where $D(\cdot, \cdot)$ is a distance measure in the embedding. $x_+$ is an
% instance in the same class as $x$ and $x_-$ is another instance in a different
% class from $x$. $m, m' \in \mathbb{R}_+$ are margins.

% Recently,
% \cite{deepRanking, facenet} adopted a triplet (inter and intra class pairs) to
% train an embedding for image similarity and face identification respectively.

% The loss function derived from the Eq.~\ref{eq:pairwise-constraints} is
% referred to as a {\bf contrastive loss}

% and a loss function derived from
% Eq.~\ref{eq:triplet-constraint} is referred to as a {\bf triplet loss}.

